Pyridyl-functionalized tripod molecules on Au(111): Interplay between H-bonding and metal coordination

The self-assembly of pyridyl-functionalized triazine (T4PT) was studied on Au(111) using low-temperature scanning tunneling microscopy (STM) under ultra-high vacuum conditions combined with density functional theory (DFT) calculations. In particular, we investigated the effect of temperature on the intermolecular interactions within the assemblies. STM measurements revealed that T4PT molecules form a well-ordered, close-packed structure, with the molecules adopting a planar conformation parallel to the Au surface for coverages $\leq1$ monolayer upon room temperature deposition. The intermolecular interactions stabilizing the self-assembled arrangement is based on a combination of hydrogen bonding and weak van der Waals forces. Upon post-deposition annealing, the assemblies are additionally stabilized by metal-ligand bonding between the pyridyl ligands and native Au adatoms. Further post-deposition annealing at temperatures above $200^{\circ}$C led to the breaking of the N-Au bonds with the molecular assemblies transforming into a second close-packed hydrogen bonded structure. For temperatures exceeding $230^{\circ}$C, few covalently linked dimers formed, most likely as a result of CH-bond activation. We rationalize the kinetically-driven structure formation by unveiling the interaction strengths of the bonding motifs using DFT and compare the molecular conformation to the structurally similar pyridyl-functionalized benzene (T4PB).

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
